Compile, Don't Memorize: A Context Compilation Architecture (CCA) for In-Context Learning

Large language models (LLMs) increasingly handle in-context learning (ICL) tasks where a long, novel context defines the rules, knowledge, and output schema for a series of questions. On benchmarks that grade against every detail of the context, even strong open-weights models pass only 12-16% of tasks: a single overlooked rule fails the whole response. We argue this brittleness is structural: the dominant "read-and-reason" paradigm asks the model to extract, plan, generate, and self-verify in one forward pass. We therefore ask whether explicit context compilation can fix it, how it compares to existing long-context strategies (gist retrieval, multi-agent self-play), and where the resulting harness benefit holds across task structure and model scale. We propose the Context Compilation Architecture (CCA), whose central novelty is a typed intermediate representation (IR) with fixed slots (rules.{must_do, must_not, conditional}, output_spec, available_tools, data_profile) into which any prose context is compiled once; executable verifiers and a violation-gated correction loop follow as downstream consequences. On CL-bench (1,899 tasks across 4 open base models), CCA outperforms vanilla prompting and two long-context baselines (ReadAgent-P, Ctx2Skill) on every base model, lifting Kimi K2.5 from 15.4% to 21.4% with gains concentrated on rule-dense sub-categories. Code and cached completions are available at https://github.com/TonyQJH/cca-emnlp2026.

==> figures/fig_subcat_lifts.tex <==
% Figure 2: per-sub-category lift of CCA over Vanilla across the four
% paper base models.  PDF generated by make_fig_subcat_lifts.py in this
% folder.  Spans both columns since 18 rows × 4 bars each does not
% compress comfortably to a single column.
\begin{figure*}[t]
\centering
\includegraphics[width=0.75\textwidth]{figures/fig_subcat_lifts_img.pdf}
\caption{\textbf{Per-sub-category lift of CCA over Vanilla, across the four base models.}
Each row is one of CL-bench's 18 sub-categories (parent domain shown in brackets and as the row's background tint: DKR, RSA, PTE, EDS); each bar gives the percentage-point pass-rate lift of CCA over Vanilla on the same (model, sub-category) cell.
Rows are sorted top-to-bottom by mean lift across the four models.
Rule-dense sub-categories cluster at the top---RSA Legal \& Regulatory (+21 to +27pp), DKR Management (+11 to +25pp), DKR Legal Advisory and RSA Programming Syntax---and show \emph{positive lifts on every model}.
Open-ended sub-categories cluster at the bottom---DKR Finance and RSA Game Mechanics underperform Vanilla on all four models by $\sim$$-9$ to $-14$pp; EDS Observational Data and PTE Instructional Procedures show similar reversals.
This is the empirical basis for the task-structural-density moderator discussed in §\ref{sec:rq3-answer}: CCA's compiled IR aligns the model toward rubric-relevant content where the context \emph{does} specify a rule system, but acts as a Procrustean bed where the context is open-ended.}
\label{fig:subcat_lifts}
\end{figure*}

